Similarity of Classification Tasks

Recent advances in meta-learning has led to remarkable performances on several few-shot learning benchmarks. However, such success often ignores the similarity between training and testing tasks, resulting in a potential bias evaluation. We, therefore, propose a generative approach based on a variant of Latent Dirichlet Allocation to analyse task similarity to optimise and better understand the performance of meta-learning. We demonstrate that the proposed method can provide an insightful evaluation for meta-learning algorithms on two few-shot classification benchmarks that matches common intuition: the more similar the higher performance. Based on this similarity measure, we propose a task-selection strategy for meta-learning and show that it can produce more accurate classification results than methods that randomly select training tasks.

==> VI.tex <==
\section{Optimise ELBO}
	\label{apdx:elbo_optimisation}
	    \subsection{Variational parameter for categorical distribution of \texorpdfstring{\(\mathbf{z}\)}{}}
    		Note that \(\mathbf{r}_{dcn}\) is a \(K\)-dimensional vector parameterized for a categorical distribution. Hence, one constrain for \(\mathbf{r}_{dcn}\) is:
    		\begin{equation}
    		    \sum_{k=1}^{K} r_{dcnk} = 1.
    		\end{equation}
    		
    		We form the Lagrangian which consists of the lower-bound with isolating terms relating \(r_{dcnk}\) and add the appropriate Lagrange multiplier:
    		\begin{equation}
    			\begin{aligned}[b]
    				\mathsf{L}[r_{dcnk}] & = \mathbb{E}_{q} \left[ \ln p(\mathbf{z} \vert \bm{\theta}) + \ln p(\mathbf{x} \vert \mathbf{z}, \bm{\mu}, \bm{\Lambda}) -\ln q(\mathbf{z}) \right] + \zeta \left(\sum_{k=1}^{K} r_{dcnk} - 1\right) \\
    				& = \frac{r_{dcnk}}{2} \left[ \ln \Tilde{\Lambda}_{k} - \nu_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k})^{\top} \mathbf{W}_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k}) - D \kappa_{k}^{-1} -D\ln(2\pi)  \right] \\
    				& \qquad + r_{dcnk} \ln \Tilde{\theta}_{dck} - r_{dcnk} \ln r_{dcnk} + \zeta \left(\sum_{k=1}^{K} r_{dcnk} - 1\right),
    			\end{aligned}
    		\end{equation}
    		where: \(\ln \Tilde{\theta}_{dck}\) and \(\ln \Tilde{\Lambda}_{k}\) are defined in Eqs.~\eqref{eq:log_tilde_theta} and \eqref{eq:log_tilde_Lambda}.
    		
    		Taking the derivative w.r.t. \(r_{dcnk}\) gives:
    		\begin{equation}
    			\begin{aligned}[b]
    				\frac{\partial \mathsf{L}}{\partial r_{dcnk}} & = \ln \Tilde{\theta}_{dck} + \frac{1}{2} \left[ \ln \Tilde{\Lambda}_{k} - \nu_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k})^{\top} \mathbf{W}_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k}) - D \kappa_{k}^{-1} -D\ln(2\pi)  \right] \\
    				& \quad - \ln r_{dcnk} - 1 + \zeta.
    			\end{aligned}
    		\end{equation}
    		
    		Setting this derivative to zero and solving for \(r_{dcnk}\) gives:
    		\begin{equation}
    		\boxed{
    			r_{dcnk} \propto \exp \left\{ \ln \Tilde{\theta}_{dck} + \frac{1}{2} \left[ \ln \Tilde{\Lambda}_{k} - \nu_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k})^{\top} \mathbf{W}_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k}) - D \kappa_{k}^{-1}  \right] \right\}.
    		}
    		    \label{eq:r}
    		  %  \tag{\ref{eq:r}}
    		\end{equation}
    	
    	\subsection{Variational parameter for Dirichlet distribution of \texorpdfstring{\(\theta\)}{}}
    		The lower-bound with isolating terms relating to only \(\gamma_{dck}\) is:
    		\begin{equation}
    			\begin{aligned}[b]
    				\mathsf{L}[\gamma_{dck}] & = \mathbb{E}_{q} \left[ \ln p(\mathbf{z} \vert \bm{\theta}) + \ln p(\bm{\theta} \vert \mathbf{y}, \bm{\alpha}) - \ln q(\bm{\theta}) \right] \\
    				& = \sum_{n=1}^{N} \sum_{k=1}^{K} r_{dcnk} \ln \Tilde{\theta}_{dck} + \sum_{l=1}^{L} \eta_{dcl} \sum_{k=1}^{K} (\alpha_{lk} - 1) \ln \Tilde{\theta}_{dck} \\
    				& \qquad + \ln B(\bm{\gamma}_{dc}) - \sum_{k=1}^{K} (\gamma_{dck} - 1) \ln \Tilde{\theta}_{dck} \\
    				& = \sum_{k=1}^{K} \ln \Tilde{\theta}_{dck} \left[\sum_{n=1}^{N} r_{dcnk} + \sum_{l=1}^{L} \eta_{dcl} (\alpha_{lk} - 1) -\gamma_{dck} + 1 \right] + \ln B(\bm{\gamma}_{dc}),
    			\end{aligned}
    		\end{equation}
    		where \(B(\mathbf{u})\) is defined in Eq.~\eqref{eq:log_dirichlet_normalized_const} -- the normalizing constant of the Dirichlet distribution parameterized by \(\mathbf{u}\).
    		
    		Taking derivative w.r.t. \(\gamma_{dck}\) gives:
    		\begin{equation}
    			\begin{aligned}[b]
    				\frac{\partial L[\gamma_{dck}]}{\partial \gamma_{dck}} & = \Psi(\gamma_{dck}) \left[\sum_{n=1}^{N} r_{dcnk} + \sum_{l=1}^{L} \eta_{dcl} (\alpha_{lk} - 1) -\gamma_{dck} + 1 \right] \\
    				& \quad - \Psi \left( \sum_{j=1}^{K} \gamma_{dcj} \right) \sum_{j=1}^{K} \left[\sum_{n=1}^{N} r_{dcnj} + \sum_{l=1}^{L} \eta_{dcl} (\alpha_{lj} - 1) -\gamma_{dcj} + 1 \right].
    			\end{aligned}
    		\end{equation}
    		Setting the derivative to zero and solve for \(\gamma_{dck}\) yields:
    		\begin{equation}
    		\boxed{
    			\gamma_{dck} = 1 + \sum_{n=1}^{N} r_{dcnk} + \sum_{l=1}^{L} \eta_{dcl} (\alpha_{lk} - 1).
    		}
    		    \label{eq:gamma}
    		  %  \tag{\ref{eq:gamma}}
    		\end{equation}
    	
    	\subsection{Variational parameter for \texorpdfstring{\(\mathbf{y}\)}{}}
    		Note that the \(L\)-dimensional vector \(\bm{\eta}_{dc}\) is the parameter of a categorical distribution for \(\mathbf{y}_{dc}\), it satisfies the following constrain:
    		\begin{equation}
    			\sum_{l=1}^{L} \eta_{dcl} = 1.
    		\end{equation}
    		The Lagrangian can be expressed as:
    		\begin{equation}
    			\begin{aligned}[b]
    				\mathsf{L}[\mathbf{y}_{dc}] & = \sum_{l=1}^{L} \eta_{dcl} \left[ - \ln B(\bm{\alpha}_{l}) + \sum_{k=1}^{K} (\alpha_{lk} - 1) \ln \Tilde{\theta}_{dck} \right] \\
    				& \quad + \sum_{l=1}^{L} \eta_{dcl} \ln \Tilde{\phi}_{dl} - \sum_{l=1}^{L} \eta_{dcl} \ln \eta_{dcl} + \xi \left(\sum_{l=1}^{L} \eta_{dcl} - 1\right).
    			\end{aligned}
    		\end{equation}
    		Taking the derivative w.r.t. \(\eta_{dcl}\) gives:
    		\begin{equation}
    			\begin{aligned}[b]
    				\frac{\partial \mathsf{L}}{\partial \eta_{dcl}} & = - \ln B(\bm{\alpha}_{l}) + \sum_{k=1}^{K} (\alpha_{lk} - 1) \ln \Tilde{\theta}_{dck} + \psi \left( \lambda_{dl} \right) - \psi \left( \sum_{j=1}^{K} \lambda_{dl} \right) - \ln \eta_{dcl} - 1 + \xi.
    			\end{aligned}
    		\end{equation}
    		Setting the derivative to zero and solve for \(\eta_{dcl}\) yields:
    		\begin{equation}
    		\boxed{
    			\eta_{dcl} \propto \exp \left[ \ln \Tilde{\phi}_{dl} - \ln B(\bm{\alpha}_{l}) + \sum_{k=1}^{K} (\alpha_{lk} - 1) \ln \Tilde{\theta}_{dck} \right].
    		}
    		    \label{eq:eta}
    		  %  \tag{\ref{eq:eta}}
    		\end{equation}
    	
    	\subsection{\texorpdfstring{Variational parameter for \(\bm{\phi}\)}{}}
    		\begin{equation}
    			\begin{aligned}[b]
    				\mathsf{L}[\bm{\lambda}_{d}] & = \sum_{c=1}^{C} \sum_{l=1}^{L} \eta_{dcl} \ln \Tilde{\phi}_{dl} + \sum_{l=1}^{L} (\delta_{l} - 1) \ln \Tilde{\phi}_{dl} + \ln B(\bm{\lambda}_{d}) - \sum_{l=1}^{L} (\lambda_{dl} - 1) \ln \Tilde{\phi}_{dl} \\
    				& = \ln B(\bm{\lambda}_{d}) + \sum_{l=1}^{L} \ln \Tilde{\phi}_{dl} \left( \delta_{l} - \lambda_{dl} + \sum_{c=1}^{C} \eta_{dcl} \right).
    			\end{aligned}
    		\end{equation}
    		Taking derivative gives:
    		\begin{equation}
    			\begin{aligned}[b]
    				\frac{\partial \mathsf{L}}{\partial \lambda_{dl}} & = \Psi(\lambda_{dl}) \left( \delta_{l} - \lambda_{dl} + \sum_{c=1}^{C} \eta_{dcl} \right) - \Psi \left(\sum_{j=1}^{L} \lambda_{dj}\right) \sum_{l=1}^{L} \left( \delta_{l} - \lambda_{dl} + \sum_{c=1}^{C} \eta_{dcl} \right).
    			\end{aligned}
    		\end{equation}
    		
    		Setting to zero and solving for \(\lambda_{dl}\) gives:
    		\begin{equation}
    		\boxed{
    			\lambda_{dl} = \delta_{l} + \sum_{c=1}^{C} \eta_{dcl}.
    		}
    		    \label{eq:lambda}
    		  %  \tag{\ref{eq:lambda}}
    		\end{equation}
    		
    	\subsection{Variational parameter for word-topics}
    		The lower-bound with the terms relating only to \(\bm{\mu}_{k}, \bm{\Lambda}_{k}\) is:
    		\begin{equation}
    			\begin{aligned}[b]
    				\mathsf{L}[\bm{\mu, \Lambda}] & = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} \sum_{k=1}^{K} \frac{r_{dcnk}}{2} \left[ \ln \Tilde{\Lambda}_{k} - \nu_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k})^{\top} \mathbf{W}_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k}) - \frac{D}{\kappa_{k}} \right] \\
    				& \quad - \sum_{k=1}^{K} \frac{1}{2} \left[ \nu_{k} \kappa_{0} (\mathbf{m}_{k} - \mathbf{m}_{0})^{\top} \mathbf{W}_{k} (\mathbf{m}_{k} - \mathbf{m}_{0}) + \frac{D \kappa_{0}}{\kappa_{k}} + D \ln \kappa_{k} \right] \\
    				& \quad - D_{\mathrm{KL}} \left[\mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \Vert \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{0}, \nu_{0} \right)\right].
    			\end{aligned}
    		\end{equation}
    		Note that:
    		\begin{align}
    			\frac{\partial}{\partial \mathbf{W}_{k}} \ln \Tilde{\Lambda}_{k} & = \left(\mathbf{W}_{k}^{-1}\right)^{\top} = \mathbf{W}_{k}^{-1} \\
    			\frac{\partial}{\partial \nu_{k}} \ln \Tilde{\Lambda}_{k} & = \frac{1}{2} \sum_{i=1}^{D} \Psi \left(\frac{\nu_{k} - i + 1}{2}\right),
    		\end{align}
    		and:
    		\begin{equation}
    			\begin{aligned}[b]
    				& D_{\mathrm{KL}} \left[\mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \Vert \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{0}, \nu_{0} \right) \right] \\
    				& = \mathcal{H} \left[\mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right), \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{0}, \nu_{0} \right)\right] - \mathcal{H} \left[\mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right)\right] \\
    				& = - \frac{\nu_{0}}{2} \ln \left| \mathbf{W}_{0}^{-1} \mathbf{W}_{k} \right| + \frac{\nu_{k}}{2} \left[\mathrm{tr}\left(\mathbf{W}_{0}^{-1} \mathbf{W}_{k}\right) - D \right] + \ln \Gamma_{D} \left(\frac{\nu_{0}}{2}\right) - \ln \Gamma_{D} \left(\frac{\nu_{k}}{2}\right)\\
    				& \qquad + \frac{\nu_{k} - \nu_{0}}{2} \psi_{D} \left(\frac{\nu_{k}}{2}\right),
    			\end{aligned}
    		\end{equation}
    		where: \(\Gamma_{D}\) and \(\psi_{D}\) are the multivariate gamma and digamma function.
    		
    		Therefore:
    		\begin{equation}
    			\begin{dcases}
    				\frac{\partial}{\partial \mathbf{W}_{k}} D_{\mathrm{KL}} & = -\frac{\nu_{0}}{2} \mathbf{W}_{k}^{-1} + \frac{\nu_{k}}{2} \mathbf{W}_{0}^{-1} \\
    				\frac{\partial}{\partial \nu_{k}} D_{\mathrm{KL}} & = \mathrm{tr}\left(\mathbf{W}_{0}^{-1} \mathbf{W}_{k}\right) - D + \frac{\nu_{k} - \nu_{0}}{4} \Psi_{D} \left(\frac{\nu_{k}}{2}\right).
    			\end{dcases}
    		\end{equation}
    		
    		Taking derivative of the lower-bound w.r.t. the variational parameters of \(\bm{\mu}_{k}, \bm{\Lambda}_{k}\) gives:
    		\begin{equation}
    				\frac{\partial \mathsf{L}}{\partial \mathbf{m}_{k}} = \nu_{k} \kappa_{0} \mathbf{W}_{k} (\mathbf{m}_{0} - \mathbf{m}_{k}) + \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} r_{dcnk}\nu_{k} \mathbf{W}_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k}).
    		\end{equation}
    		\begin{equation}
    			\begin{aligned}[b]
    				\frac{\partial \mathsf{L}}{\partial \kappa_{k}} = \frac{D \kappa_{0}}{2 \kappa_{k}^{2}} - \frac{D}{2 \kappa_{k}} + \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} \frac{D r_{dcnk}}{2 \kappa_{k}^{2}} = \frac{D}{2\kappa_{k}^{2}} \left[\kappa_{0} - \kappa_{k} + \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} r_{dcnk} \right].
    			\end{aligned}
    		\end{equation}
    		\begin{equation}
    			\begin{aligned}[b]
    				\frac{\partial \mathsf{L}}{\partial \mathbf{W}_{k}} & = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} \frac{r_{dcnk}}{2} \left[ \mathbf{W}_{k}^{-1} - \nu_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k})^{\top} (\mathbf{x}_{dcn} - \mathbf{m}_{k}) \right] \\
    				& \quad -\frac{1}{2} \nu_{k} \kappa_{0} (\mathbf{m}_{k} - \mathbf{m}_{0})^{\top} (\mathbf{m}_{k} - \mathbf{m}_{0}) + \frac{\nu_{0}}{2} \mathbf{W}_{k}^{-1} - \frac{\nu_{k}}{2} \mathbf{W}_{0}^{-1}.
    			\end{aligned}
    		\end{equation}
    		\begin{equation}
    			\begin{aligned}[b]
    				\frac{\partial \mathsf{L}}{\partial \nu_{k}} & = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} \frac{r_{dcnk}}{2} \left[ \frac{1}{2} \sum_{i=1}^{D} \Psi \left(\frac{\nu_{k} - i + 1}{2}\right) - (\mathbf{x}_{dcn} - \mathbf{m}_{k})^{\top} \mathbf{W}_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k}) \right] \\
    				& \quad - \frac{1}{2} \kappa_{0} (\mathbf{m}_{k} - \mathbf{m}_{0})^{\top} \mathbf{W}_{k} (\mathbf{m}_{k} - \mathbf{m}_{0}) \\
    				& \quad - \mathrm{tr}\left(\mathbf{W}_{0}^{-1} \mathbf{W}_{k}\right) + D - \frac{\nu_{k} - \nu_{0}}{4} \Psi_{D} \left(\frac{\nu_{k}}{2}\right).
    			\end{aligned}
    		\end{equation}
    		
    		Setting these partial derivatives to zero and solving for the 4 parameters of interest give:
    		\begin{equation}
    		\boxed{
    		    \begin{aligned}[b]
        			\mathbf{m}_{k} & = \frac{\kappa_{0}}{\kappa_{0} + N_{k}} \mathbf{m}_{0} + \frac{N_{k}}{\kappa_{0} + N_{k}} \bar{\mathbf{x}}_{k} \\
        			\kappa_{k} & = \kappa_{0} + N_{k} \\
        			\mathbf{W}_{k}^{-1} & = \mathbf{W}_{0}^{-1} + N_{k} \mathbf{S}_{k} + \frac{\kappa_{0} N_{k}}{\kappa_{0} + N_{k}} (\bar{\mathbf{x}}_{k} - \mathbf{m}_{0}) (\bar{\mathbf{x}}_{k} - \mathbf{m}_{0})^{\top} \\
        			\nu_{k} & = \nu_{0} + N_{k},
    			\end{aligned}
    		}
    			\label{eq:m_step}
                % \tag{\ref{eq:m_step}}
    		\end{equation}
    		where:
    % 		\begin{align}
    % 			N_{k} & = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} r_{dcnk} \tag{\ref{eq:Nk}} \\
    % 			\bar{\mathbf{x}}_{k} & = \frac{1}{N_{k}} \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} r_{dcnk} \mathbf{x}_{dcn} \tag{\ref{eq:xbar_k}} \\
    % 			\mathbf{S}_{k} & = \frac{1}{N_{k}} \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} r_{dcnk} (\mathbf{x}_{dcn} - \bar{\mathbf{x}}_{k}) (\mathbf{x}_{dcn} - \bar{\mathbf{x}}_{k})^{\top}. \tag{\ref{eq:Sk}}
    % 		\end{align}
    		\begin{align}
			N_{k} & = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} r_{dcnk} \label{eq:Nk} \\
			\bar{\mathbf{x}}_{k} & = \frac{1}{N_{k}} \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} r_{dcnk} \mathbf{x}_{dcn} \label{eq:xbar_k} \\
			\mathbf{S}_{k} & = \frac{1}{N_{k}} \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} r_{dcnk} (\mathbf{x}_{dcn} - \bar{\mathbf{x}}_{k}) (\mathbf{x}_{dcn} - \bar{\mathbf{x}}_{k})^{\top}. \label{eq:Sk}
		\end{align}
		
	\input{learning_algorithm}
    	
    \section{Detail derivation of each term in ELBO}
	\label{apdx:elbo_derivation}
	
		\subsection{\texorpdfstring{\(\mathbb{E}_{q} \left[\ln p(\mathbf{z} \vert \bm{\theta}) \right] \)}{}}
			\begin{equation}
				\begin{aligned}[b]
					\mathbb{E}_{q} \left[\ln p(\mathbf{z} \vert \bm{\theta}) \right] & = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} \sum_{k=1}^{K} q(z_{dcnk} = 1; \mathbf{r}_{dcn}) \, \int q(\bm{\theta}_{dc}; \bm{\gamma}_{dc}) \ln p(z_{dcnk} = 1 \vert \bm{\theta}_{dc}) \, d\bm{\theta}_{dc} \\
					& = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} \sum_{k=1}^{K} r_{dcnk} \, \int \mathrm{Dir}_{K} \left( \bm{\theta}_{dc}; \bm{\gamma}_{dc} \right) \, \ln \theta_{dck} \, d\bm{\theta}_{dck} \\
					& = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} \sum_{k=1}^{K} r_{dcnk} \ln \Tilde{\theta}_{dck},
				\end{aligned}
			\end{equation}
			where:
			\begin{equation}
				\ln \Tilde{\theta}_{dck} = \psi \left( \gamma_{dck} \right) - \psi \left( \sum_{j=1}^{K} \gamma_{dcj} \right).
				\label{eq:log_tilde_theta}
				% \tag{\ref{eq:log_tilde_theta}}
			\end{equation}
			
		\subsection{\texorpdfstring{\(\mathbb{E}_{q} \left[\ln p(\bm{\theta} \vert \mathbf{y}, \bm{\alpha}) \right] \)}{}}
			\begin{equation}
				\begin{aligned}[b]
					\mathbb{E}_{q} \left[\ln p(\bm{\theta} \vert \mathbf{y}, \bm{\alpha}) \right] & = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{l=1}^{L} q(y_{dcl} = 1; \bm{\eta}_{dc}) \int q(\bm{\theta}_{dc}; \bm{\gamma}_{dc}) \, \ln p( \bm{\theta}_{dc} \vert y_{dcl} = 1, \bm{\alpha}) \, d\bm{\theta}_{dc} \\
					& = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{l=1}^{L} \eta_{dcl} \int \mathrm{Dir}_{K} (\bm{\theta}_{dc}; \bm{\gamma}_{dc}) \, \ln \mathrm{Dir}_{K} ( \bm{\theta}_{dc}; \bm{\alpha}_{l}) \, d\bm{\theta}_{dc}.
				\end{aligned}
			\end{equation}
			Note that the cross-entropy between 2 Dirichlet distributions can be expressed as:
			\begin{equation}
			\begin{aligned}[b]
			\mathcal{H} \left[\mathrm{Dir} \left(\mathbf{x}; \bm{\alpha}_{0}\right), \mathrm{Dir} \left(\mathbf{x}; \bm{\alpha}_{1} \right) \right] & = - \mathbb{E}_{\mathrm{Dir} \left(\mathbf{x}; \bm{\alpha}_{0} \right)} \left[ \ln \mathrm{Dir} \left(\mathbf{x}; \bm{\alpha}_{1} \right) \right] \\
			& = - \mathbb{E}_{\mathrm{Dir} \left(\mathbf{x}; \bm{\alpha}_{0} \right)}  \left[ - \ln B(\bm{\alpha_{1}}) + \sum_{k=1}^{K} (\alpha_{1k} - 1) \ln x_{k} \right] \\
			& = \ln B(\bm{\alpha}_{1}) - \sum_{k=1}^{K} (\alpha_{1k} - 1) \left[ \psi(\alpha_{0k}) - \psi \left( \sum_{k^{\prime}=1}^{K} \alpha_{0k^{\prime}} \right) \right],
			\end{aligned}
			\end{equation}
			where:
			\begin{equation}
				\ln B(\bm{\alpha}_{1}) = \sum_{k=1}^{K} \ln\Gamma \left( \alpha_{1k} \right) - \ln\Gamma \left( \sum_{j=1}^{K} \alpha_{1j} \right).
				\label{eq:log_dirichlet_normalized_const}
				% \tag{\ref{eq:log_dirichlet_normalized_const}}
			\end{equation}
			Hence:
			\begin{equation}
    			\begin{aligned}[b]
                    \mathbb{E}_{q} \left[\ln p(\bm{\theta} \vert \mathbf{y}, \bm{\alpha}) \right] & = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{l=1}^{L} \eta_{dcl} \left[ - \ln B(\bm{\alpha}_{l}) + \sum_{k=1}^{K} (\alpha_{lk} - 1) \ln \Tilde{\theta}_{dck} \right].
    			\end{aligned}
			\end{equation}
			
		\subsection{\texorpdfstring{\(\mathbb{E}_{q} \left[\ln p(\mathbf{y} \vert \bm{\phi}) \right] \)}{}}
			\begin{equation}
				\begin{aligned}[b]
					\mathbb{E}_{q} \left[\ln p(\mathbf{y} \vert \bm{\phi}) \right] & = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{l=1}^{L} q(y_{dcl} = 1; \bm{\eta}_{dc}) \int q(\bm{\phi}_{d}; \bm{\lambda}_{d}) \ln p(y_{dcl} = 1 \vert \bm{\phi}_{d}) \, d\phi_{d} \\
					& = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{l=1}^{L} \eta_{dcl} \int \mathrm{Dir} (\bm{\phi}_{d}; \bm{\lambda}_{d}) \ln \phi_{dl} \, d\phi_{d} \\
					& = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{l=1}^{L} \eta_{dcl} \ln \Tilde{\phi}_{dl},
				\end{aligned}
			\end{equation}
			where:
			\begin{equation}
			    \ln \Tilde{\phi}_{dl} = \psi \left( \lambda_{dl} \right) - \psi \left( \sum_{j=1}^{K} \lambda_{dl} \right)
			    \label{eq:log_tilde_phi}
			 %   \tag{\ref{eq:log_tilde_phi}}
			\end{equation}
		
		\subsection{\texorpdfstring{\(\mathbb{E}_{q} \left[\ln p(\bm{\phi} \vert \bm{\delta}) \right] \)}{}}
			\begin{equation}
				\begin{aligned}[b]
					\mathbb{E}_{q} \left[\ln p(\bm{\phi} \vert \bm{\delta}) \right] & = \sum_{d=1}^{M} \int q(\bm{\phi}_{d}; \bm{\lambda}_{d}) \ln p(\bm{\phi}_{d} \vert \bm{\delta}) \, d\bm{\phi}_{d} \\
					& = \sum_{d=1}^{M} \int \mathrm{Dir}_{L} (\bm{\phi}_{d}; \bm{\lambda}_{d}) \ln \mathrm{Dir}_{L} (\bm{\phi}_{d} \vert \bm{\delta}) \, d\bm{\phi}_{d} \\
					& = \sum_{d=1}^{M} \ln \frac{\Gamma \left(\sum_{l=1}^{L} \delta_{l}\right)}{\prod_{l=1}^{L} \Gamma \left(\delta_{l}\right)} + \sum_{l=1}^{L} (\delta_{l} - 1) \ln \Tilde{\phi}_{dl}.
				\end{aligned}
			\end{equation}
			
		\subsection{\texorpdfstring{\(\mathbb{E}_{q} \left[\ln p(\mathbf{x} \vert \mathbf{z}, \bm{\mu}, \bm{\Lambda}) \right] \)}{}}
			\begin{equation}
				\begin{aligned}[b]
					& \mathbb{E}_{q} \left[\ln p(\mathbf{x} \vert \mathbf{z}, \bm{\mu}, \bm{\Lambda}) \right] \\
					& = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} \sum_{k=1}^{K} q(z_{dcnk} = 1; \mathbf{r}_{dcn}) \\
					& \qquad \times \int q(\bm{\mu}_{k}, \bm{\Lambda}_{k}; \mathbf{m}_{k}, \kappa_{k}, \mathbf{W}_{k}, \nu_{k}) \ln p(\mathbf{x}_{dcn} \vert z_{dcnk} = 1, \bm{\mu}, \bm{\Lambda})  \, d\bm{\mu} \, d\bm{\Lambda} \\
					& = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} \sum_{k=1}^{K} r_{dcnk} \\
					& \qquad \times \int \mathcal{N} \left(\bm{\mu}_{k}; \mathbf{m}_{k}, \left(\kappa_{k} \bm{\Lambda}_{k} \right)^{-1} \right) \, \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \ln \mathcal{N}(\mathbf{x}_{dcn} \vert \bm{\mu}_{k}, \bm{\Lambda}_{k}^{-1})  \, d\bm{\mu}_{k} \, d\bm{\Lambda}_{k} \\
					& = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} \sum_{k=1}^{K} \frac{r_{dcnk}}{2} \int \mathcal{N} \left(\bm{\mu}_{k}; \mathbf{m}_{k}, \left(\kappa_{k} \bm{\Lambda}_{k} \right)^{-1} \right) \, \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \times \\
					& \qquad \qquad \times \left[\ln |\bm{\Lambda}_{k}| - (\mathbf{x}_{dcn} - \bm{\mu}_{k})^{\top} \bm{\Lambda}_{k} (\mathbf{x}_{dcn} - \bm{\mu}_{k}) -D \ln(2\pi)  \right]  \, d\bm{\mu}_{k} \, d\bm{\Lambda}_{k} \\
				\end{aligned}
			\end{equation}
			Note that:
			\begin{equation}
				\ln \Tilde{\Lambda}_{k} = \int \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \ln |\bm{\Lambda}_{k} | \, d\bm{\Lambda}_{k} = \sum_{i=1}^{D} \psi \left(\frac{\nu_{k} - i + 1}{2}\right) + D \ln (2) + \ln |\mathbf{W}_{k} |,
				\label{eq:log_tilde_Lambda}
				% \tag{\ref{eq:log_tilde_Lambda}}
			\end{equation}
			and
			
			\begin{equation}
				\begin{aligned}[b]
					& \mathbb{E}_{\bm{\mu}_{k}} \left[ (\mathbf{x}_{dcn} - \bm{\mu}_{k})^{\top} \bm{\Lambda}_{k} (\mathbf{x}_{dcn} - \bm{\mu}_{k}) \right] \\
					& = \mathbb{E}_{\bm{\mu}_{k}} \left[ (\mathbf{x}_{dcn} - \mathbf{m}_{k})^{\top} \bm{\Lambda}_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k}) + (\mathbf{x}_{dcn} - \mathbf{m}_{k})^{\top} \bm{\Lambda}_{k} (\mathbf{m}_{k} - \bm{\mu}_{k}) \right. \\
					& \qquad \left. + (\mathbf{m}_{k} - \bm{\mu}_{k})^{\top} \bm{\Lambda} (\mathbf{x}_{dcn} - \mathbf{m}_{k}) + (\mathbf{m}_{k} - \bm{\mu}_{k})^{\top} \bm{\Lambda} (\mathbf{m}_{k} - \bm{\mu}_{k}) \right] \\
					& = (\mathbf{x}_{dcn} - \mathbf{m}_{k})^{\top} \bm{\Lambda}_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k}) + \mathbb{E}_{\bm{\mu}_{k}} \left[ (\mathbf{m}_{k} - \bm{\mu}_{k})^{\top} \bm{\Lambda} (\mathbf{m}_{k} - \bm{\mu}_{k}) \right] \\
					& = (\mathbf{x}_{dcn} - \mathbf{m}_{k})^{\top} \bm{\Lambda}_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k}) + \mathrm{tr} \left[ \bm{\Lambda} \mathbb{E}_{\bm{\mu}_{k}} \left[ (\mathbf{m}_{k} - \bm{\mu}_{k})^{\top} (\mathbf{m}_{k} - \bm{\mu}_{k}) \right] \right] \\
					& = (\mathbf{x}_{dcn} - \mathbf{m}_{k})^{\top} \bm{\Lambda}_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k}) + \mathrm{tr} \left[ \bm{\Lambda} \left(\kappa_{k} \bm{\Lambda}_{k}\right)^{-1} \right] \\
					& = (\mathbf{x}_{dcn} - \mathbf{m}_{k})^{\top} \bm{\Lambda}_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k}) + D \kappa_{k}^{-1}
				\end{aligned}
			\end{equation}
			\begin{equation}
				\begin{aligned}[b]
					\Rightarrow \mathbb{E}_{\bm{\mu}_{k}, \bm{\Lambda}_{k}} \left[ (\mathbf{x}_{dcn} - \bm{\mu}_{k})^{\top} \bm{\Lambda}_{k} (\mathbf{x}_{dcn} - \bm{\mu}_{k}) \right] & = \mathbb{E}_{\bm{\mu}_{k}, \bm{\Lambda}_{k}} \left[ (\mathbf{x}_{dcn} - \mathbf{m}_{k})^{\top} \bm{\Lambda}_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k}) + D \kappa_{k}^{-1} \right] \\
					& = \nu_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k})^{\top} \mathbf{W}_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k}) + D \kappa_{k}^{-1}.
				\end{aligned}
			\end{equation}
			Hence:
			\begin{equation}
				\begin{aligned}[b]
					\mathbb{E}_{q} \left[\ln p(\mathbf{x} \vert \mathbf{z}, \bm{\mu}, \bm{\Lambda}) \right] & = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} \sum_{k=1}^{K} \frac{r_{dcnk}}{2} \left[ \ln \Tilde{\Lambda}_{k} - D \kappa_{k}^{-1} -D\ln(2\pi)  \vphantom{\frac{1}{2}} - \right.\\
					& \qquad \left. - \nu_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k})^{\top} \mathbf{W}_{k} (\mathbf{x}_{dcn} - \mathbf{m}_{k}) \right]
				\end{aligned}
			\end{equation}
			
		\subsection{\texorpdfstring{\(\mathbb{E}_{q} \left[\ln p(\bm{\mu}, \bm{\Lambda} \vert \mathbf{m}_{0}, \kappa_{0}, \mathbf{W}_{0}, \nu_{0})\right] \)}{}}
			\begin{equation}
				\begin{aligned}[b]
					& \mathbb{E}_{q} \left[\ln p(\bm{\mu}, \bm{\Lambda} \vert \mathbf{m}_{0}, \kappa_{0}, \mathbf{W}_{0}, \nu_{0})\right] \\
					& = \sum_{k=1}^{K} \int \mathcal{N} \left(\bm{\mu}_{k}; \mathbf{m}_{k}, \left(\kappa_{k} \bm{\Lambda}_{k} \right)^{-1} \right) \, \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \\
					& \qquad \times \ln \left[ \mathcal{N} \left(\bm{\mu}_{k}; \mathbf{m}_{0}, \left(\kappa_{0} \bm{\Lambda}_{k} \right)^{-1} \right) \, \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{0}, \nu_{0} \right) \right] d\bm{\mu}_{k} \, d\bm{\Lambda}_{k} \\
					& = \sum_{k=1}^{K} \int \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \left[ \int \mathcal{N} \left(\bm{\mu}_{k}; \mathbf{m}_{k}, \left(\kappa_{k} \bm{\Lambda}_{k} \right)^{-1} \right) \, \ln \mathcal{N} \left(\bm{\mu}_{k}; \mathbf{m}_{0}, \left(\kappa_{0} \bm{\Lambda}_{k} \right)^{-1} \right) d\bm{\mu}_{k} \right] d\bm{\Lambda}_{k} \\
					& \qquad + \int \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \, \ln \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{0}, \nu_{0} \right) d\bm{\Lambda}_{k}.
				\end{aligned}
			\end{equation}
			Note that:
			\begin{equation}
				\begin{aligned}[b]
					& \int \mathcal{N} \left(\bm{\mu}_{k}; \mathbf{m}_{k}, \left(\kappa_{k} \bm{\Lambda}_{k} \right)^{-1} \right) \, \ln \mathcal{N} \left(\bm{\mu}_{k}; \mathbf{m}_{0}, \left(\kappa_{0} \bm{\Lambda}_{k} \right)^{-1} \right) d\bm{\mu}_{k} \\
					& = -\frac{1}{2} \int \mathcal{N} \left(\bm{\mu}_{k}; \mathbf{m}_{k}, \left(\kappa_{k} \bm{\Lambda}_{k} \right)^{-1} \right) \\
					& \qquad \times \left[ D \ln (2\pi) - D \ln \kappa_{0} - \ln |\bm{\Lambda}_{k}| + \kappa_{0} (\bm{\mu}_{k} - \mathbf{m}_{0})^{\top} \bm{\Lambda}_{k} (\bm{\mu}_{k} - \mathbf{m}_{0}) \right] d\bm{\mu}_{k} \\
					& = \frac{1}{2} \left[ D \ln \left(\frac{\kappa_{0}}{2\pi}\right)  + \ln | \bm{\Lambda}_{k} | - \kappa_{0} (\mathbf{m}_{k} - \mathbf{m}_{0})^{\top} \bm{\Lambda}_{k} (\mathbf{m}_{k} - \mathbf{m}_{0}) - \frac{D \kappa_{0}}{\kappa_{k}} \right]
				\end{aligned}
			\end{equation}
			\begin{equation}
				\begin{aligned}[b]
					\Rightarrow & \int \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \left[ \int \mathcal{N} \left(\bm{\mu}_{k}; \mathbf{m}_{k}, \left(\kappa_{k} \bm{\Lambda}_{k} \right)^{-1} \right) \, \ln \mathcal{N} \left(\bm{\mu}_{k}; \mathbf{m}_{0}, \left(\kappa_{0} \bm{\Lambda}_{k} \right)^{-1} \right) d\bm{\mu}_{k} \right] d\bm{\Lambda}_{k} \\
					& = \frac{1}{2} \left[ D \ln \left(\frac{\kappa_{0}}{2\pi}\right) + \ln \Tilde{\Lambda}_{k} - \nu_{k} \kappa_{0} (\mathbf{m}_{k} - \mathbf{m}_{0})^{\top} \mathbf{W}_{k} (\mathbf{m}_{k} - \mathbf{m}_{0}) - \frac{D \kappa_{0}}{\kappa_{k}} \right]
				\end{aligned}
			\end{equation}
			and the cross-entropy between 2 Wishart distributions can be written as:
			\begin{equation}
				\begin{aligned}[b]
					& \int \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \, \ln \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{0}, \nu_{0} \right) d\bm{\Lambda}_{k} = - \mathcal{H} \left[(\mathbf{W}_{k}, \nu_{k}), (\mathbf{W}_{0}, \nu_{0})\right] \\
					& = \frac{\nu_{0}}{2} \ln \left| \mathbf{W}_{0}^{-1} \mathbf{W}_{k} \right| - \frac{D + 1}{2} \ln \left| \mathbf{W}_{k} \right| - \frac{\nu_{k}}{2} \mathrm{tr} \left( \mathbf{W}_{0}^{-1} \mathbf{W}_{k} \right) - \log \Gamma_{D} \left( \frac{\nu_{0}}{2} \right) +\\
					& \qquad + \frac{\nu_{0} - D - 1}{2} \psi_{D} \left( \frac{\nu_{k}}{2} \right) - \frac{D (D + 1)}{2} \ln (2)\\
					& = - \frac{\nu_{0}}{2} \ln \left| \mathbf{W}_{0} \right| + \frac{\nu_{0} - D - 1}{2} \left[ \psi_{D} \left( \frac{\nu_{k}}{2} \right) + \ln \left| \mathbf{W}_{k} \right| + D \ln(2) \right] - \frac{\nu_{k}}{2} \mathrm{tr} \left( \mathbf{W}_{0}^{-1} \mathbf{W}_{k} \right) -\\
					& \quad - \log \Gamma_{D} \left( \frac{\nu_{0}}{2} \right) - \frac{\nu_{0} D}{2} \ln (2) \\
					& = -\frac{\nu_{0}}{2} \ln \left| \mathbf{W}_{0} \right| + \frac{\nu_{0} - D - 1}{2} \ln \Tilde{\Lambda}_{k} - \frac{\nu_{k}}{2} \mathrm{tr} \left( \mathbf{W}_{0}^{-1} \mathbf{W}_{k} \right) - \log \Gamma_{D} \left( \frac{\nu_{0}}{2} \right) - \frac{\nu_{0} D}{2} \ln (2),
				\end{aligned}
			\end{equation}
			where \(\Gamma_{D}(.)\) and \(\psi_{D}(.)\) are the multivariate gamma and digamma functions, respectively.
			
			Hence, the expectation of interest can be expressed as:
			\begin{equation}
				\begin{aligned}[b]
					& \mathbb{E}_{q} \left[\ln p(\bm{\mu}, \bm{\Lambda} \vert \mathbf{m}_{0}, \kappa_{0}, \mathbf{W}_{0}, \nu_{0})\right] \\
					& = \sum_{k=1}^{K} \frac{1}{2} \left[ D \ln \left(\frac{\kappa_{0}}{2\pi}\right) + \ln \Tilde{\Lambda}_{k} - \nu_{k} \kappa_{0} (\mathbf{m}_{k} - \mathbf{m}_{0})^{\top} \mathbf{W}_{k} (\mathbf{m}_{k} - \mathbf{m}_{0}) - \frac{D \kappa_{0}}{\kappa_{k}} \right] - \\
					& \quad -\frac{\nu_{0}}{2} \ln \left| \mathbf{W}_{0} \right| + \frac{\nu_{0} - D - 1}{2} \ln \Tilde{\Lambda}_{k} - \frac{\nu_{k}}{2} \mathrm{tr} \left( \mathbf{W}_{0}^{-1} \mathbf{W}_{k} \right) - \log \Gamma_{D} \left( \frac{\nu_{0}}{2} \right) - \frac{\nu_{0} D}{2} \ln (2).
				\end{aligned}
			\end{equation}
			The result is identical to the previous derivation in the literature \cite[Eq.~(10.74)]{bishop2006pattern}.
		
		\subsection{\texorpdfstring{\(\mathbb{E}_{q} \left[\ln q(\mathbf{z})\right] \)}{}}
			\begin{equation}
				\begin{aligned}[b]
					\mathbb{E}_{q} \left[\ln q(\mathbf{z})\right] & = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{n=1}^{N} \sum_{k=1}^{K} r_{dcnk} \ln r_{dcnk}.
				\end{aligned}
			\end{equation}
		
		\subsection{\texorpdfstring{\(\mathbb{E}_{q} \left[\ln q(\bm{\theta})\right] \)}{}}
			\begin{equation}
				\begin{aligned}[b]
					\mathbb{E}_{q} \left[\ln q(\bm{\theta})\right] & = - \sum_{d=1}^{M} \sum_{c=1}^{C} \ln B(\bm{\gamma}_{dc}) - \sum_{j=1}^{K} (\gamma_{dck} - 1) \ln \Tilde{\theta}_{dck}.
				\end{aligned}
			\end{equation}
		
		\subsection{\texorpdfstring{\(\mathbb{E}_{q} \left[\ln q(\mathbf{y})\right] \)}{}}
			\begin{equation}
				\mathbb{E}_{q} \left[\ln q(\mathbf{y})\right] = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{l=1}^{L} \eta_{dcl} \ln \eta_{dcl}.
			\end{equation}
		
		\subsection{\texorpdfstring{\(\mathbb{E}_{q} \left[\ln q(\bm{\phi})\right] \)}{}}
			\begin{equation}
				\begin{aligned}[b]
					\mathbb{E}_{q} \left[\ln q(\bm{\phi})\right] & = - \sum_{d=1}^{M} \ln B(\bm{\lambda}_{d}) - \sum_{l=1}^{L} (\lambda_{dl} - 1) \ln \Tilde{\phi}_{dl}.
				\end{aligned}
			\end{equation}
		
		\subsection{\texorpdfstring{\(\mathbb{E}_{q} \left[\ln q(\bm{\mu, \Lambda})\right] \)}{}}
			\begin{equation}
				\begin{aligned}[b]
					& \mathbb{E}_{q} \left[ \ln q(\bm{\mu, \Lambda}) \right] \\
					& = \sum_{k=1}^{K} \mathbb{E}_{q(\bm{\mu}_{k}, \bm{\Lambda}_{k})} \left[ \ln q(\bm{\mu}_{k}, \bm{\Lambda}_{k}) \right] \\
					& = \sum_{k=1}^{K} \int \mathcal{N} \left(\bm{\mu}_{k}; \mathbf{m}_{k}, (\kappa_{k} \bm{\Lambda}_{k})^{-1} \right) \, \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \left[ \ln \mathcal{N} \left(\bm{\mu}_{k}; \mathbf{m}_{k}, (\kappa_{k} \bm{\Lambda}_{k})^{-1} \right) \right. \\
					& \qquad \left. + \ln \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \right] d\bm{\mu}_{k} \, d\bm{\Lambda}_{k} \\
					& = \sum_{k=1}^{K} \int \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \left[ \int \mathcal{N} \left(\bm{\mu}_{k}; \mathbf{m}_{k}, (\kappa_{k} \bm{\Lambda}_{k})^{-1} \right) \ln \mathcal{N} \left(\bm{\mu}_{k}; \mathbf{m}_{k}, (\kappa_{k} \bm{\Lambda}_{k})^{-1} \right) \, d\bm{\mu}_{k} \right] d\bm{\Lambda}_{k} \\
					& \qquad + \int \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \ln \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \, d\bm{\Lambda}_{k} \\
					& = - \sum_{k=1}^{K} \int \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right) \frac{1}{2} \ln | 2\pi e (\kappa_{k} \bm{\Lambda}_{k})^{-1} | \, d\bm{\Lambda}_{k} + \mathcal{H} \left[\mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right), \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right)\right] \\
					& = \sum_{k=1}^{K} \left\{ \frac{1}{2} \ln \Tilde{\Lambda}_{k} + \frac{D}{2} \ln \left( \frac{\kappa_{k}}{2\pi} \right) - \frac{D}{2} - \mathcal{H} \left[\mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right), \mathcal{W} \left( \bm{\Lambda}_{k}; \mathbf{W}_{k}, \nu_{k} \right)\right] \right\}.
				\end{aligned}
			\end{equation}
	
    \section{Experiments on Omniglot and mini-ImageNet}
    \label{apdx:experiment_details}
        For Omniglot, we follow the pre-processing steps as in few-shot image classification without any data augmentation, and use the standard train-test split in the original paper to prevent information leakage. For mini-ImageNet, we follow the common train-test split with 80 classes for training and 20 classes for testing~\cite{ravi2017optimization}. Since the dimension of raw images in mini-ImageNet is large, we employ the 640-dimensional features extracted from a wide-residual-network~\cite{rusu2019meta} to ease the calculation.
    
        We follow Algorithm~\ref{alg:online_ldcc} to obtain the parameters of the image-topics posterior using tasks in training set. We use \(L = 8\) task-topics and \(K = 16\) image-topics for Omniglot, and \(L = 3\) and \(K = 10\) for mini-ImageNet. The Dirichlet distribution for task-topic proportion is chosen to be symmetric with \(\delta = 0.01\). The hyper-parameter \(\bm{\alpha}\) is uniformly chosen in \([0.01, 0.1]\) and held fixed in each experiment. The training for LDCC is carried out with 20 images per class to fit into the memory of a Nvidia 1080 Ti GPU, while the inference of the variational parameter \(\bm{\lambda}\) is done on all available labelled data in each class (\(20\) for Omniglot and \(600\) for mini-ImageNet). Note that this is for the inference of LDCC used in the correlation diagram. For the task selection, this number matches the number of shots in the few-shot learning setting.
        
        \subsection{Pre-processing}
            For Omniglot, the grey-scale images of each character are resized to 28-by-28 pixels, resulting in a 728-dimensional vector. We use the original train-test split, where 30 alphabets are used for training, and the other 20 alphabets are used for testing. No rotation is applied to augment classes.
            
            For mini-ImageNet, we use the extracted features that are presented by 640-dimensional vectors. In addition, we normalise those features to be within [0, 1] by multiplying with a factor of 3.
        
        \subsection{Hyper-parameters in LDCC}
            The prior parameters of image-topics, \(\mathbf{m}_{0}, \kappa_{0}, \mathbf{W}_{0}, \nu_{0}\), are selected as follows:
            \begin{itemize}
                \item The mean \(\mathbf{m}_{0}\) is selected as the mean of all the images in the training of each data set,
                \item \(\kappa_{0}\) is set to \(0.01\),
                \item The scale matrix \(\mathbf{W}_{0}\) is selected as the covariance matrix of all the images in the training set,
                \item \(\nu_{0}\) is set to the dimension of images (728 for Omniglot and 640 for mini-ImageNet) adding 2.
            \end{itemize}
            
            The hyper-parameters for the learning rate used in online learning are \(\tau_{0} = 100\) and \(\tau_{1} = 0.5\). The mini-batch used in both data sets for LDCC is \(500\).
            
        \subsection{Network architectures used in meta-learning}
            We use two different network architectures on the two data sets. For Omniglot, we follow the \say{standard} 4 module CNN network, where each module consists of 64 3-by-3 filter convolutional layer, followed by batch normalisation, activated by ReLU and 2-by-2 max-pooling. For mini-ImageNet, we use a fully connected network with 1 hidden layer consisting of 128 hidden units, activated by ReLU.
            
    \section{Infer Dirichlet parameters \texorpdfstring{\(\bm{\alpha}\)}{alpha}}
    \label{apdx:alpha}
        The terms in ELBO which contains \(\bm{\alpha}\) are:
        \begin{equation}
            \begin{aligned}[b]
                \mathsf{L}[\bm{\alpha}] & = \sum_{d=1}^{M} \sum_{c=1}^{C} \sum_{l=1}^{L} \eta_{dcl} \left[ \ln\Gamma\left(\sum_{k=1}^{K} \alpha_{lk}\right) - \sum_{k=1}^{K} \ln\Gamma\left(\alpha_{lk}\right) + \sum_{k=1}^{K} (\alpha_{lk} - 1) \ln \Tilde{\theta}_{dck} \right].
            \end{aligned}
        \end{equation}
        
        Taking the derivative w.r.t. \(\alpha_{lk}\) gives:
        \begin{equation}
            \begin{aligned}
                \frac{\partial \mathsf{L}}{\partial \alpha_{lk}} & = g_{lk} =  M \left[ \psi \left(\sum_{k=1}^{K} \alpha_{lk}\right) - \psi\left(\alpha_{lk}\right) \right] \sum_{c=1}^{C} \eta_{dcl}  + \sum_{d=1}^{M} \sum_{c=1}^{C} \eta_{dcl} \ln \Tilde{\theta}_{dck}.
            \end{aligned}
        \end{equation}
        
        The Hessian matrix can be calculated as:
        \begin{equation}
            \begin{aligned}
                \frac{\partial^{2} \mathsf{L}}{\partial \alpha_{lk} \partial\alpha_{lj}} & = \underbrace{M \left[ \sum_{c=1}^{C} \eta_{dcl} \right] \Psi \left(\sum_{k=1}^{K} \alpha_{lk}\right)}_{u} \, \underbrace{- M \left[ \sum_{c=1}^{C} \eta_{dcl} \right] \mathbbm{1}[k = j] \, \Psi\left(\alpha_{lk}\right)}_{q_{ljk}}.
            \end{aligned}
        \end{equation}
        
        According to \cite{minka2000estimating}, Newton-Raphson method can be used to infer \(\bm{\alpha}_{l}\) as:
        \begin{align}
            \bm{\alpha}_{l} & \gets \bm{\alpha}_{l} - \mathbf{H}_{l}^{-1} \mathbf{g}_{l} \\
            \mathbf{H}_{l}^{-1} & = \mathbf{Q}_{l}^{-1} - \frac{\mathbf{Q}_{l}^{-1} \mathbf{11}^{\top} \mathbf{Q}_{l}^{-1}}{1 / u + \mathbf{1}^{\top} \mathbf{Q}_{l}^{-1} \mathbf{1}} \\
            \left(\mathbf{H}_{l}^{-1} \mathbf{g}_{l} \right)_{l} & = \frac{g_{lk} - b_{l}}{q_{lkk}},
        \end{align}
        where:
        \begin{equation}
            \begin{aligned}
                    b_{l} & = \frac{\mathbf{1}^{\top} \mathbf{Q}_{l}^{-1} \mathbf{g}_{l}}{1 / u + \mathbf{1}^{\top} \mathbf{Q}_{l}^{-1} \mathbf{1}} = \frac{\sum_{j} g_{lj} q_{ljj}}{1 / u + \sum_{j} 1 / q_{ljj}}.
            \end{aligned}
        \end{equation}

==> review_from_nips.tex <==
\section{Review from Neurips 2020}
    \textbf{Insufficient evaluation for the task selection, e.g. adding a baseline, varying the number of ways and the number of training examples.} Originally, we only ran the experiment shown in \figureautorefname{~\ref{fig:task_selection}} without the baseline Task2Vec and fixing the setting for 5-way 5-shot. In the current version, we add more experiments as shown in \figureautorefname{~\ref{fig:varying_num_tasks_ways}} with several variations in term of number of classes within a task, and the number of training tasks. The baseline Task2Vec is also included in the comparison.
    
    \textbf{The proposed approach adds an inefficient step.} The proposed approach is not about meta-learning, but to learn a generative model to represent tasks in an embedding space. The obtained representation can be used either for task similarity (as presented in the paper) or further downstream transfer-learning works, such as task augmentation. Here, we use it as a pre-processing step before performing meta-learning for demonstration purpose without claiming its efficiency. If considering such applications, other baselines, such as Task2Vec, also share the same computational burden when calculating task-to-task distances.
    
    \textbf{Is the proposed approach restricted to gradient based meta-learning algorithms?}
    Meta-learning is used to demonstrate the concept of task similarity quantification proposed in our paper, so our method is not restricted to any particular meta-learning algorithm. To demonstrate that, the submitted paper shows the results using the metric-based Prototypical Networks (we replicate the paper results in Fig.~\ref{fig:protonet_5way} and add the 10-way result in Fig.~\ref{fig:protonet_10way}). The extension to other meta-learning algorithms is trivial.
    
    \textbf{Experimenting on only 2 data sets.}
    The reason for using those two data sets is that the our proposed approach works with low-dimensional data (Omniglot) or extracted features (mini-ImageNet). We will demonstrate our method on other data sets by embedding images into a lower-dimensional embedding space before performing LDCC. The training at that stage will be to learn both the image embedding and LDCC simultaneously.
